Towards a Rigorous Evaluation of XAI Methods on Time Series

Explainable Artificial Intelligence (XAI) methods are typically deployed to explain and debug black-box machine learning models. However, most proposed XAI methods are black-boxes themselves and designed for images. Thus, they rely on visual interpretability to evaluate and prove explanations. In this work, we apply XAI methods previously used in the image and text-domain on time series. We present a methodology to test and evaluate various XAI methods on time series by introducing new verification techniques to incorporate the temporal dimension. We further conduct preliminary experiments to assess the quality of selected XAI method explanations with various verification methods on a range of datasets and inspecting quality metrics on it. We demonstrate that in our initial experiments, SHAP works robust for all models, but others like DeepLIFT, LRP, and Saliency Maps work better with specific architectures.

==> content/concept.tex <==
\clearpage

\section{Concept Introduction}
\begin{itemize}
    \item Introduction to XAI
    \begin{itemize}
        \item AI usage everywhere
        \item EU law of interpretability
        \item Need for XAI
    \end{itemize}
    \item Motivation for XAI methods
    \begin{itemize}
        \item Trust Building
        \item Debugging / Refinement
        \item Fairness Proofing
        \item Privacy Proofing
    \end{itemize}
    \item Time Series Applications as a Use Case and new challenge
    \begin{itemize}
        \item Predictive Maintenance
        \item Heartbeat Anomaly Detection
        \item High-Frequency Trade Forecasting
        \item Electric Power Consumption
        \item More: Sound Classification / Shape Classification / ...
    \end{itemize}
    \item \textbf{Definitions}:
    \begin{itemize}
        \item \textbf{XAI Method}: XAI Algorithm to be applied on model
        \item \textbf{XAI Explainer}: XAI method used on to model and its output
        \item \textbf{XAI Explanation}: Explainer is visualized or verbalized
    \end{itemize}
    \item Challenges of XAI methods on Time Series
    \begin{itemize}
        \item Tested in most cases only on images.
        \item Which XAI method works on TS?
        \item Which XAI method generates an explainer?
        \item Which XAI explainer generates an explanation?
        \item What is a suitable explanation on time series?
        \item Do we need to abstract time series to form explanations?
        \item What is a suitable abstraction to generate explanations?
    \end{itemize}
\end{itemize}

\section{Definitions of XAI method criteria}

\begin{itemize}
    \item XAI TS method criteria
    \begin{itemize}
        \item 
    \end{itemize}
    \item Table of properties
    \begin{itemize}
        \item See Tab: \ref{tab:tsporp}
    \end{itemize}
\end{itemize}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|}
\hline
Model-agnostic vs model-specific & \begin{tabular}[c]{@{}l@{}}Model agnostic XAI methods focus on the input and output of a model\\   and can be applied onto every possible machine learning model, some example\\   methods: LIME, PDP, …\\   \\   \\   Model specific XAI methods only work on certain model types, like\\   Neural Networks, e.g. LRP, Saliency\end{tabular}                                                  \\ \hline
Local vs global                  & \begin{tabular}[c]{@{}l@{}}Local XAI methods focus on explanations on the basis of samples and\\   through that explains a decision making for the sample, e.g. LIME.\\   \\   \\   Global XAI methods try to explain the whole model decision making\\   without the need of certain samples. In some cases, the whole training\\   dataset is needed, e.g. Trepan / RuleMatrix.\end{tabular} \\ \hline
Types of Explanation    & \begin{tabular}[c]{@{}l@{}}XAI method produces explanation on the model input space and show\\   which input is important for certain outputs, e.g. Feature Importance, LIME,\\   …\\    \\   XAI method produces explanation on an abstraction of the model input\\   space based e.g. on descriptive features\end{tabular}                                                                   \\ \hline
Degree of Approximation of Explainers         & \begin{tabular}[c]{@{}l@{}}XAI method shows uncertainty in its output, e.g. RuleMatrix on the\\   discrepancy between surrogate model and real model\end{tabular}\\\hline                           
\end{tabular}
\caption{Table showing the different TS XAI method properties. The last two will either be quite sparse or answered only as the same for most of the current XAI methods. This highlights the current research question. \newline \blue{Is there enough explanation? What needs more?}}
\label{tab:tsporp}
\end{table*}



\section{Evaluation of XAI methods}

\subsection{\textbf{Methodology}}



\begin{itemize}
    \item \textbf{Requirement Analysis}
    \begin{itemize}
        \item Different wide spread Time Series datasets to show range of applicability
        \item Show applicability of various XAI methods
    \end{itemize}
    \item \textbf{Task Analysis}
    \begin{itemize}
        \item Show dataset differences
        \item Use XAI methods on many datasets
        \item Show that XAI methods produce output
        \item Show that XAI methods produce explanation
    \end{itemize}
    \item \textbf{Goal Analysis}
    \begin{itemize}
        \item Categorize XAI methods into not working, not useful, useful
        \item Categorize produced explanation into not meaningful, meaningful
    \end{itemize}
    \item \textbf{Need for Quality Metrics on explanations}
    \begin{itemize}
        \item \textbf{How to categorize explanations into different groups such as useful, meaningful, etc.}
        \item \blue{What is the distinction between working, useful, meaningful?}
        \item \blue{Which meaningful to tackle? Based on ML Expert, Domain Expert, Non-Expert}
        \item \blue{Is meaningful heavily task dependent?}
        \item \blue{Do we need meaningful explanations or useful explanations?}
        \item \blue{Do understanding, diagnosis and refinement need different meaningful definitions?}
        \item \blue{Is there an interaction between them?}
    \end{itemize}
    \item \textbf{Evaluation Description}
    \begin{itemize}
        \item Take Dataset and proposed model for it
        \item Use different XAI methods on it
        \item Store results of XAI methods
        \item Analyze produced XAI method explanation
    \end{itemize}
\end{itemize}

\subsection{Systematic Dimensions}
\begin{itemize}
    \item \textbf{Dataset / Data task}
    \item \textbf{Model / Model parameters}
    \item \textbf{XAI method / XAI method parameters}
\end{itemize}

\begin{figure}[htb]
  \includegraphics[width=\linewidth]{data/SystematicTest.PNG}
  \caption{Systematic Dimensions.}
  \label{fig:dimensions}
\end{figure}

\subsection{Evaluation}

\subsubsection{\textbf{Dataset and data task systematic exploration}}
\begin{itemize}
    \item Classification
    \begin{itemize}
        \item Human Activity Recognition
    \end{itemize}
    \item Anomaly Detection / Outlier Detection
    \begin{itemize}
        \item Heartbeat
    \end{itemize}
    \item Forecasting
    \begin{itemize}
        \item Stock Market Prediction
    \end{itemize}
\end{itemize}

\subsubsection{\textbf{Model and parameters exploration}}
\begin{itemize}
    \item \textbf{Dataset benchmark model}
    \item Convolution Neural Network
    \item Recurrent Neural Network
    \item Alternative Models
    \begin{itemize}
        \item ARIMA / HA
        \item Linear / Polynomic / Possion Regression
    \end{itemize}
\end{itemize}

\subsubsection{\textbf{XAI method and parameters exploration}}
\begin{itemize}
    \item \textbf{LIME}
    \begin{itemize}
        \item Tabular Method
        \begin{itemize}
            \item Change Kernel Size
            \item Change sample number
        \end{itemize}
        \item Image Method
        \begin{itemize}
            \item Change superpixel number
            \item Change sample number
        \end{itemize}
    \end{itemize}
    \item \textbf{LRP}
    \begin{itemize}
        \item Change epsilon
    \end{itemize}
    \item \textbf{Saliency Maps}
    \begin{itemize}
        \item Change modifiers
    \end{itemize}
    \item \textbf{SHAP}
    \begin{itemize}
        \item Kernel Method
        \begin{itemize}
            \item Change sample number
        \end{itemize}
        \item Deep Method
        \begin{itemize}
            \item Rank outputs
        \end{itemize}
        \item Gradient Method
        \begin{itemize}
            \item Change smoothing
        \end{itemize}
        \item Linear Method
        \begin{itemize}
            \item Change sample number
            \item Change feature dependency
        \end{itemize}
    \end{itemize}
    \item \textbf{CAV}
    \begin{itemize}
        \item Concepts
        \item Change number of concepts
    \end{itemize}
\end{itemize}

\blue{Are there more dimensions to explore?}

\section{Guidelines and Research Gaps}

\begin{itemize}
    \item \textbf{Guidelines for explanations on TS}
    \begin{itemize}
        \item Which work and how meaningful are these
        \item Which explanation fits which task
        \item Recommend one to use for one task, but also some other possibilities
    \end{itemize}
    \item \textbf{Research Gaps towards a good solution for XAI methods on TS}
    \begin{itemize}
        \item \textbf{More human-readable abstraction for explanations}
        \item More meaningful explanations
        \item Easier to use XAI methods
        \item Suit XAI method to task and problem
    \end{itemize}
\end{itemize}

\section{Conclusions}

\begin{itemize}
    \item Summarize and conclude
    \item Repeat key points
    \item Propose important criteria
\end{itemize}

\begin{itemize}
    \item \red{Towards descriptive features used together with feature importance}
\end{itemize}


\section*{Figures:}

\begin{figure}[htb]
  \includegraphics[width=\linewidth]{data/HeartbeatData.PNG}
  \caption{Heartbeat Data for each category. Blue category N. Orange category S. Green category V. Red category F. Violet category Q. Y-Axis: Amplitude of normalized data, X-Axis: Time.}
  \label{fig:heartbeat}
\end{figure}

\begin{figure}[htb]
  \includegraphics[width=\linewidth]{data/Lime.PNG}
  \caption{LIME importance (red background - the darker the background color the more important the feature or time-point is for the sample to be classified as the category) for one sample (blue) and class mean (green).}
  \label{fig:lime}
\end{figure}

\begin{figure}[htb]
  \includegraphics[width=\linewidth]{data/Shap.PNG}
  \caption{Top: SHAP Deep method for one samples. Every feature shows a weight towards the predicted score. Blue corresponds to worsen the result for this sample. Red means it improves the result for this sample. Bottom: SHAP deep method for classes. Feature or in our case time-point importance for the different classes. Feature 2 and 3 are very important for the class 0 or category N.}
  \label{fig:shap}
\end{figure}

==> content/current_status.tex <==

\section*{Done so far:}

\begin{enumerate}
    \item Crawled and loaded heartbeat data
    \begin{itemize}
        \item Crawled heartbeat data
        \item Loaded data
        \item Cleaned data
        \item Preprocessed data
    \end{itemize}
    \item Visualized heartbeat data
    \begin{itemize}
        \item Plotted data for each category See Fig. \ref{fig:heartbeat}
        \item Calculated mean of it
        \item Plotted both into single plot
    \end{itemize}
    \item Explored heartbeat data
    \begin{itemize}
        \item Explored relationship mean of class to class samples
        \item Explored mean of classes to each other
    \end{itemize}
    \item Rebuild heartbeat classification paper model
    \begin{itemize}
        \item Rebuild in Keras the proposed Deep Learning Model for this dataset
        \item Changed some unclear optimizations
    \end{itemize}
    \item Trained classification model
    \begin{itemize}
        \item Trained DNN on the heartbeat data with the proposed parameters for batch size
        \item Stopped after 50 epochs due to convergence
    \end{itemize}
    \item Inspected classification model
    \begin{itemize}
        \item Inspected accuracy of model on data
        \item Interesting high accuracy on data
    \end{itemize}
    \item Applied LIME on model
    \begin{itemize}
        \item Build pipeline to incorporate LIME
        \item Used LIME tabular explainer
        \item Trained LIME explainer with default values on data
    \end{itemize}
    \item Explored LIME explanation
    \begin{itemize}
        \item Plotted LIME explanation as list and rank them based on their importance
        \item Plotted LIME result into previous data plot
        \item Inpsected plot and heatmap over the time series data See Fig. \ref{fig:lime}
    \end{itemize}
    \item Applied SHAP kernel method on model
    \begin{itemize}
        \item Changed data to fit SHAP kernel method
        \item Plot for one sample to explain
        \item Plot for every sample of the test to explain
    \end{itemize}
    \item Applied SHAP deep method on model
    \begin{itemize}
        \item Changed data to fit SHAP deep method
        \item Plot for one sample to explain
        \item Plot for every sample of the test to explain See Fig. \ref{fig:shap}
    \end{itemize}
    \item Explored SHAP explanations
    \begin{itemize}
        \item Explored both methods against each other
        \item Found some strange findings between both methods 
    \end{itemize}
    \item Created decision tree to verify some explanations
    \begin{itemize}
        \item Trained decision tree on data to explore if feature important for LIME and SHAP are important as a split criteria
        \item Dismissed decision tree idea as it was not useful
    \end{itemize}
    \item Brought this all into an experiment environment
    \begin{itemize}
        \item Rewrite all into some environment to automatically do it for various datasets and explore the results afterwards
    \end{itemize}
    \item Applied LRP on it
    \begin{itemize}
        \item LRP has some problems with various architectures
        \item Works in general but not for RNNs
    \end{itemize}
    \item Applied DeepLift on it
    \begin{itemize}
        \item DeepLift has some problems with various architectures
        \item Works in general but not for some layer types
    \end{itemize}
    \item Applied Saliency Maps on it
    \begin{itemize}
        \item Saliency Maps works for nearly all architecture types
        \item Has some performance issues
    \end{itemize}
    \item Applied SHAP on it
    \begin{itemize}
        \item Rewrote SHAP output to be used in the same way as heatmaps before
        \item SHAP is quite slow
    \end{itemize}
    \item Applied SHAP on it
    \begin{itemize}
        \item Rewrote SHAP output to be used in the same way as heatmaps before
        \item SHAP is quite slow
    \end{itemize}
    \item Create own time importance algorithm
    \begin{itemize}
        \item First implement feature importance with time points as features
        \item Extend it to a general time importance version
    \end{itemize}
\end{enumerate}

\section*{Next up:}

\begin{enumerate}
    \item Improve own time importance algorithm
    \begin{itemize}
        \item Runtime is way too worse
        \item Needs to be speed up
        \item Some sampling should help
    \end{itemize}
    \item Create own feature abstraction XAI algorithm
    \begin{itemize}
        \item Abstractly 
    \end{itemize}
\end{enumerate}





==> content/paper/Z-old-text.tex <==
%%%% 2

% Other fields like computer vision
% Due to complex models, such as CNNs or RNNs, achieve state-of-the-art performance on various tasks, more and more traditional and interpretable models get exchanged with Deep Neural Networks (DNN).
% However, these DNNs are hardly understandable in their decision making and need additional XAI methods on top of them to explain themselves.
% Especially, explaining the outcomes of classifiers has a heavy usage in computer vision tasks to verify the correctness of various object recognition tasks.
% Debugging models, e.g., autonomous driving to harden them and make them more robust against adversarial attacks is a crucial task to develop safe autonomous cars.
% Further, increasing trust in a model is another critical task to convince users even to use a specific model.

% Time Series more difficult
% Images and text are in an XAI explanation context easier to explain as they already incorporate human knowledge by visualizing data quickly.
% A classification of a dog with a visualization of an XAI explanation heatmap showing the nose and ears as necessary for the prediction has a heavy bias to be a correct explanation for a user.
% Text classification, which highlights certain words a human would combine to the class, also enables the same bias.
% Time series, on the other hand, are hard to visualize and are hardly understood by domain experts in many cases.
% Often, experts need abstract representations such as frequency transformations to be able to work with time-series data.
% Thus, XAI explanations of time series are more difficult to interpret and need to be verified by a quantifiable method at first.
